Constraints on Weak Supernova Kicks from Observed Pulsar Velocities

Observations of binary pulsars and pulsars in globular clusters suggest that at least some pulsars must receive weak natal kicks at birth. If all pulsars received strong natal kicks above \unit[50]{\kms}, those born in globular clusters would predominantly escape, while wide binaries would be disrupted. On the other hand, observations of transverse velocities of isolated radio pulsars indicate that only $5\pm2\%$ have velocities below \unit[50]{\kms}. We explore this apparent tension with rapid binary population synthesis modelling. We propose a model in which supernovae with characteristically low natal kicks (e.g., electron-capture supernovae) only occur if the progenitor star has been stripped via binary interaction with a companion. We show that this model naturally reproduces the observed pulsar speed distribution and without reducing the predicted merging double neutron star yield. We estimate that the zero-age main sequence mass range for non-interacting progenitors of electron-capture supernovae should be no wider than ${\approx}0.2 M_\odot$.

==> referee_response2.tex <==
===========================================
We thank the reviewers for their follow-up feedback which further improved the manuscript.  The requested change is detailed below.

-----

Reviewer #2:

I am still confused about how the authors draw low kicks for CCSN. Is it from the same Maxwellian distribution for low natal kicks used for ECSN or from the Hobbs distribution? It would be helpful to clarify this in the paper.


> We have updated the relevant section to the following: "To obtain a 3D kick magnitude for the CC-pulsars, we randomly draw a velocity sample from the union of the transverse velocity posterior distributions of pulsars in our catalogue, selecting only among values of at least \unit[50]{\kms}, and divide by a random projection coefficient under the assumption of an isotropic viewing angle."
